Collocated Adaptive Control of Underactuated Mechanical Systems

Collocated adaptive control of underactuated systems is still a main concern for the control community, all the more so because the collocated dynamics is no longer linear with respect to the constant base parameters. This work extends and encompasses the well known adaptive control result for fully actuated mechanical systems to the underactuated case. The key point is the introduction of a fictitious control input that allows us to consider the complete system dynamics, which is assumed to be linear with respect to the base parameters. Local stability and convergence of time varying reference trajectories for the collocated dynamics are demonstrated by using Lyapunov and Barbalat arguments. Simulation and experimental results on a two-link manipulator verify the soundness of the proposed approach.

==> header.tex <==

\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}

\usepackage{color,graphicx}
\usepackage{subfig}

\usepackage{ae,aecompl,bm}
\let\proof\relax
\let\endproof\relax
\usepackage[cmex10]{amsmath} % assumes amsmath package installed

\usepackage[stable]{footmisc}

% \usepackage[noadjust]{cite}
% \usepackage[sort]{natbib}
\renewcommand{\cite}{\citep}

\usepackage{enumitem,url,theorem}
\usepackage{IEEEtrantools,mathtools}
\usepackage{algorithm,algorithmic}

